Fault Tolerant Frequent Pattern Mining

FP-Growth algorithm is a Frequent Pattern Min- ing (FPM) algorithm that has been extensively used to study correlations and patterns in large scale datasets. While several researchers have designed distributed memory FP-Growth algorithms, it is pivotal to consider fault tolerant FP-Growth, which can address the increasing fault rates in large scale systems. In this work, we propose a novel parallel, algorithm-level fault-tolerant FP-Growth algorithm. We leverage algorithmic properties and MPI advanced features to guarantee an O(1) space complexity, achieved by using the dataset memory space itself for checkpointing. We also propose a recovery algorithm that can use in-memory and disk-based checkpointing, though in many cases the recovery can be completed without any disk access, and incurring no memory overhead for checkpointing. We evaluate our FT algorithm on a large scale InfiniBand cluster with several large datasets using up to 2K cores. Our evaluation demonstrates excellent efficiency for checkpointing and recovery in comparison to the disk-based approach. We have also observed 20x average speed-up in comparison to Spark, establishing that a well designed algorithm can easily outperform a solution based on a general fault-tolerant programming model.

==> Makefile <==
#
# $Id: Makefile 161 2007-11-30 07:19:52Z balaji $
#
# Copyright (C) 2006-2007, University of Chicago. All rights reserved.
#

.PHONY: all clean complete

tex_files = $(wildcard *.tex */*.tex */*/*.tex */*/*/*.tex)
bib_files = $(wildcard *.bib */*.bib */*/*.bib */*/*/*.bib)
eps_files = $(wildcard *.eps */*.eps */*/*.eps */*/*/*.eps)
epsi_files = $(wildcard *.epsi */*.epsi */*/*.epsi */*/*/*.epsi)
ps_files = $(wildcard */*.ps */*/*.ps */*/*/*.ps)

header: header.tex $(tex_files) $(bib_files)
	@if test "`which rubber `" != "" ; then \
		rubber -d header ; \
	else \
		pdflatex header | tee latex.out ; \
		if grep -q '^LaTeX Warning: Citation.*undefined' latex.out; then \
			bibtex header; \
			touch .rebuild; \
		fi ; \
		while [ -f .rebuild -o \
			-n "`grep '^LaTeX Warning:.*Rerun' latex.out`" ]; do \
			rm -f .rebuild; \
			pdflatex header | tee latex.out; \
		done ; \
		rm latex.out ; \
	fi

clean:
	find . \( -name '*.blg' -print \) -or \( -name '*.aux' -print \) -or \
		\( -name '*.bbl' -print \) -or \( -name '*~' -print \) -or \
		\( -name '*.lof' -print \) -or \( -name '*.lot' -print \) -or \
		\( -name '*.toc' -print \) | xargs rm -f; \
	rm -f header.dvi header.log header.pdf _region_* \
		summary.pdf cv_vishnu.pdf header.out


==> text/amft_old.tex <==
\subsection{Asynchronous Memory-based  Fault Tolerance (AMFT)}

Any effective fault tolerance system of parallel application should  incur  less checkpointing and failure recovery  
overheads~\cite{zheng2004ftc}. Using memory as a checkpointing storage  leads to the challenge of   space availability. In the case of large  
datasets, memory space can be an obstacle of applying a memory-based checkpointing technique. In this section, we exploit one-sided  
communication technology (MPI-RMA) features to design a robust Memory-based Fault Tolerance (AMFT) approach to handle failures in the 
parallel FP-growth algorithm.

With the observation of the memory space availability through parallel FP-growth algorithm execution,  
%% GA: the  above is not clear to me 
our proposed AMFT approach require the  same amount of memory space that is  initiated  consumed by storagte of  dataset transactions.  
Moreover, the AMFT approach design takes care of unreliable characteristic of memory as a checkpointing storing destination,  by performing  
critical checkpoint in the case of failure similar to the SMFT approach.  
%% GA: last part of above sentence is not clear - you don't take checkpoints when there is a failure? 
Finally, AMFT approach provides an asynchronous checkpointing mechanism by using MPI-RMA technology to avoid extra communication overhead, 
 which is the main limitation of SMFT approach.


\begin{figure}[H]
\centering
\psfig{figure=figs/metadata.eps,width=65mm}
\caption{Fault Tolerance Metadata Record Structure}
\label{fig:metadata}
\end{figure}


Initially, a one record meta-data structure is defined  for  each process defining several parameters and is   used by our fault tolerance  
system. This record contains six parameters: Local Samples PTR (LS-PTR), Checkpointed FP-Tree PTR (CF-PTR), Checkpointed FP-Tree Size (CFS),  
Current Transaction (CT), Start Checkpointed Transaction (SCT), and Number of Checkpointed Transactions (NCT).  Figure~\ref{fig:metadata} shows  the structure of both checkpoints and metadata-data structures of a certain process $P_i$

In AMFT, preserving the same memory space can simply be performed by using local transactions memory space as the checkpointing space.  
Assuming again a communication ring structure of $P$ processes, using MPI-RMA, each process $P_{i}$ shares  its local transactions' memory  
space and meta-data record with other processes. Each process $P_i$ updates local LS-PTR value based on the progress it accomplishes on  
processing transactions vector. This value is used to mark the beginning of the unprocessed transactions and the space available for adjacent  
process $P_{i-1}$ to checkpoint its data.
After processing a set of transactions, each process is ready to perform the first checkpoint. Three types of checkpointing process can  
be performed: complete checkpoint (i.e., local FP-Tree and remaining samples), partial checkpoint (i.e., local FP-Tree only), and 
a non-checkpoint.  
%% GA: not clear what a non-checkpoint is 
Once one complete checkpoint is performed, all the following checkpoints will be partial checkpoints. Each process $P_{i-1}$ performs  a  
certain checkpoint type based on the available memory space of the adjacent process $P_{i}$'s  local transactions vector. Using  
MPI-RMA MPI\_Get function, Process $P_{i-1}$ reads LS-PTR value of the process $P_{i}$ to decide whether to perform complete, partial,  or  
no checkpointing. This process is performed independently without any synchronization between worker processes.

In the case that  memory space is available, using MPI-RMA MPI\_PUT function, process $P_{i-1}$ copies its remaining samples (in the 
case of a  complete checkpoint) and current local FP-Tree to process $P_i$ memory. This is a non-blocking operation that can be overlapped with  
execution to hide data transfer latency.
After this, process $P_{i-1}$ remotely updates process $P_{i}$ meta-data attributes by setting  CF-PTR equals to 0 if no samples checkpointing  
has been performed or CF-PTR equals to the size of checkpointed transactions. CFS and CT are updated to current checkpointed FP-Tree size and  
current $P_{i-1}$  processed transaction, respectively. In the case of complete checkpoint, SCT and NCT is updated to the first checkpointed  
transaction on checkpointed transactions vector and the number of checkpointed transactions, respectively. Figure~\ref{fig:checkpoint} gives an overview of proposed checkpointing mechanism.


%\begin{figure}[!htb]
%\centerline{\psfig{figure=figs/checkpoint-types.eps,width=65mm} }
%\caption{AMFT Checkpointing Mechanism}
%\label{fig:checkpoint}
%\end{figure}

\begin{figure}[!htb]
\centering
  \subcaptionbox{Partial Checkpoint\label{fig:x7}}{\includegraphics[width=35mm]{figs/AMFT1.eps}}\hspace{1em}%
  \subcaptionbox{Complete Checkpoint\label{fig:x8}}{\includegraphics[width=35mm]{figs/AMFT2.eps}}\hspace{1em}%
\caption{AMFT Checkpointing Mechanism}
\label{fig:checkpoint}
\end{figure}


Time complexity of AMFT checkpointing algorithm is $\mathcal{O}(b.(C.s+T)$ per process. Because AMFT approach uses a non-blocking communication routines this time will be hidden and overlapped with the execution. Further, the space complexity of AMTF approach is $\mathcal{O}(1)$ because we use the space occupied by already processed transactions on the adjacent node's memory.


The recovery mechanism in AMFT approach is almost identical  to the SMFT recovery algorithm. Assuming a process $P_i$ fails while generating  
its local FP-Tree,  the master process informs process $P_{i+1}$ to recover the failed process. Process $P_{i+1}$ uses checkpoint parameters on  
metadata record to recover process $P_{i}$. Recovery algorithm should deal with three different cases. First, neither $P_{i}$ FP-Tree nor  
transactions have been checkpointed. In this case, the process $P_{i+1}$ reads $P_{i}$'s  transactions from the disk and redistributes them  
to the available nodes. Second, if only $P_i$'s  FP-Tree has been checkpointed, process $P_{i+1}$ will merge process $P_i$'s  checkpointed  
FP-Tree with its current local FP-Tree and, just like   the first case,  it will read and redistribute $P_i$'s  local transactions using the  
disk. Third, if both $P_i$ FP-Tree and transactions has been checkpointed, $P_i$'s  checkpointed FP-Tree and $P_{i+1}$s  FP-Trees  will be  
merged. In this case, the  disk I/O latency can be eliminated by reading the remaining unprocessed transactions from the memory and  
redistributing them to the available nodes by process $P_{i+1}$. Similar to the SMFT approach, process $P_{i-1}$ performs critical checkpoint  
on the process $P_{i+1}$ because its backup process $P_i$ already failed. Time complexity of the AMFT recovery algorithm in the case of recovering both samples and FP-Tree from memory is $\mathcal{O}(m+b.T)$.


%????????
%
%performs local FP-Tree checkpoint on process $P_{i}$ memory by accessing {\em checkpoints} space on its memory, storing its current local FP-Tree, and modifying values on {\em meta-data} data-structure.
%
%
%
%by sharing the memory space contains local transactions with other processes.
%
%
%
%
%
%. At time $t0$ process $P_{i-1}$ performs a checkpoint with size $x$ into process $P_i$ memory. The starting offset of this checkpoint,i.e 0,  is stored on $CSO$ attribute and the checkpoint size is stored on $CS$ in meta-data data structure. All the following checkpoints will keep the same structure. The space complexity of AMC checkpoint operation can be estimated as  $\mathcal{O}(P.C.(s+1))$ to store both data structures on memory. Further, the time complexity is $\mathcal{O}(C.l.(s+1))$. This time latency can be hidden using MPI-RMA technology.
%
%
%
%
%
%Asynchronous Memory-based  Checkpointing (AMC) mechanism uses MPI-RMA technology to store checkpoints in memory rather than going to disk which reduce both checkpointing and recovery overhead. Each process shares a memory space with other processes that can handle the local FP-Tree of another process during the execution to be used as a FP-Tree checkpointing space. In this case, it is important to define suitable vectors that can be used to store a neighbor process' FP-Tree.
%
%AMC approach depends on defining two vectors by each process , i.e. each with different MPI-RMA window, which should be shared with other processes: a {\em checkpoints} data-structure that holds the local FP-Trees of a specific process $P_i$, and {\em meta-data} data-structure which describes the checkpoint's metadata (i.e., Checkpointed Starting Offset (CSO), Checkpointed Size (CS), Last Processed Transaction (LPT), and Checkpoint Number(CN)).




//Stop
To summarize, there are several advantages of using AMC fault tolerance mechanism: asynchronous checkpointing technique that minimizes the total communication cost, each process only needs to handle one checkpoint of its proceeding process at a time, the ability to handle more than one processes failure, and avoid mater process bottleneck by recovering failure from different processes.
Algorithm~\ref{alg:AMFT} illustrates checkpoint/recover procedures to apply AMFT mechanism. In initialization procedure, each process create two vectors $checkpoints$ and $metadata$ and an atomic variable $TreesCheckpointOffset (TCO)$ to handle neighbors processes checkpoints (lines 1-2). In lines [2-3], Two dynamic MPI-RMA memory are defined to mange the $checkpoints$ and $metadata$ vectors , i.e., $dyn\_win\_chk $and $dyn\_win\_metadata$, and a single static window to handle $TCO$ variable ,i.e., $win\_TCO$. Both $checkpoints$ and $metadata$ vectors and $TCO$ variable are attached to created windows (lines 5-7)

$PerformLFPChk$ procedure illustrates checkpoint operation in SMFT.  Alternately, each process $p_i$ chooses its target process $TargetProcess$ to be $P_{i+1}$ or $P_{i+2}$ and similarly its source process $SrcProcess$ to be $P_{i-1}$ or $P_{i-2}$ (lines 1-6). Instantly, each process $p_i$ sends its current local FP-Tree size $L.Tree.size()$ to its $TargetProcess$ (Line 8). Therefore, the $TargetProcess$ can resize $checkpoints$ vector by $SrcTreeSize$ to be able to handle $P_i$ local FP-Tree (lines 9-10). $metadata$ vector is also resized to handle one metadata record (i.e.,CSO,CS,LPT, and CN (Figure~\ref{fig:AMC})). As an MPI-RMA requirement both $checkpoints$ and $metadata$ vectors are re-attached to their dynamic memory (line 11)). Moreover, the new MPI addresses of both two vectors are send to $src_process$ for future MPI remote memory access (lines 12-13). To prevent remote memory access collision, $TargetLTO$ variable should be updated atomically by the $srcProcess$ (line 14). After this, $SrcProcess$ checkpoints its current local FP-Tree  and updates $TargetMetadata$  on  $TargetProcess$ memory using MPI-RMA function ($MPI\_PUT$) (lines 15-16)).


Finally, $performRecovery$ procedure shows the recovery operation in SMFT. Because every process $P_i$ have two checkpoints on the system, a reduction operation is performed to recognize the process that has the latest checkpoint of the failed process $RecProcess$ (Line 1). $RecProcess$ merges its Local FP-Tree and failed process $P_f$ FP-Tree while the master process try to re-read unprocessed transaction of failed process from the disk (Lines 2-3).

\begin{algorithm} [htp]
\setstretch{1.2}
  \caption{\bf AMFT Mechanism}
\label{alg:SMFT}
\begin{algorithmic}[1]
\Require {\bf Procedure: initialization($chk\_schema$ = SMFT)}
\State Create $checkpoints$ and $metadata$ vectors (initially-empty).
\State Initiate an atomic variable $TCO$.
\State Create two dynamic memory windows $dyn\_win\_chk$ and $dyn\_win\_metadata$ \enspace {\bf(MPI\_Win\_create\_dynamic)}
\State Create a static memory window for $TCO$ variable $win\_TCO$\enspace {\bf(MPI\_Win\_create)}
\State Attach($checkpoints$, $dyn\_win\_chk$) \enspace {\bf(MPI\_Win\_attach)}
\State Attach($metadata$, $dyn\_win\_metadata$) \enspace {\bf(MPI\_Win\_attach)}
\State Attach($TCO$, $win\_TCO$) \enspace {\bf(MPI\_Win\_attach).}
\NoNumber\hrulefill
\NoNumber {\bf Procedure: performLFPChk ($L.Tree$)}
\setcounter{ALG@line}{0}
\If{$ChkIteration$\%2==0}
    \State $TargetProcess$ = $P_{i+1}$
    \State $SrcProcess$ = $P_{i-1}$
\Else
    \State $TargetProcess$ = $P_{i+2}$
    \State $SrcProcess$ = $P_{i-2}$
\EndIf

\State SendLFPTreeSize ($L.Tree.size()$, $TargetProcess$)
\State $SrcTreeSize$= ReceiveCkhSize ($L.Tree.size()$, $SrcProcess$)
\State ResizeVec ($checkpoints$, $metadata$, $SrcTreeSize$)
\State Re-attachToWin ($checkpoints$, $dyn\_win\_chk$, $metadata$, $dyn\_win\_metadata$) \enspace ({\bf MPI\_Win\_detach} and {\bf MPI\_Win\_attach})
\State SendVecAddress ($checkpoints$, $metadata$ , $SrcProcess$)
\State $TargetAddress$=RecvVecAddress ($Targetcheckpoints$, $Targetmetadata$ , $TargetProcess$)
\State $TargetLTO$=$TargetLTO$+$L.FPTree.size()$ \enspace (Atomically update using {\bf MPI\_Fetch\_and\_op})
\State Add ($L.FPTree$, $Targetcheckpoints$,$TargetAddress$) \enspace ({\bf MPI\_Put})
\State Update($Targetmetadata$) \enspace ({\bf MPI\_Put})

\NoNumber\hrulefill
\NoNumber {\bf Procedure: performRecovery ($P_f$, $G.Freq.List$)}
\setcounter{ALG@line}{0}
\State $RecProcess$=AllReduce ($metadata.CN$, $P_f$) \enspace ({\bf MPI\_Allreduce})
\NoNumber {\bf Recovery process:}
\State  merge ($L.Tree$, $P_f.chkFPTree$, $G.Freq.List$)
\NoNumber {\bf Master process:}
\State   RecUnprocessedTrans( $P_f$)
 \end{algorithmic}
\end{algorithm}


Algorithm~\ref{alg:generateLFPTree} explain the abstract view of our FT local FP-Tree generation procedure(i.e., Algorithm 1 (line 6)) using the proposed FT Fp-groth algorithms (i.e., ADC, SMFT, and ESMFT).
To generate local FP-Tree, each process merge the current transaction $T$ to local FP-Tree $L.Tree$ (line 5). Based on a pre-determine number of checkpoints, after merging a set of transactions, each process needs to perform a FP-Tree checkpoint (line 7). If $chk_schema$is a memory-based schema, each process needs to remove any invalid checkpoints it has in its memory (line 9). In the case of ESMFT mechanism, transactions checkpoint should be performed when the total number of processed transactions satisfies  equation~\ref{equation:equ4} (lines 12-13). In the case of failure and memory-based FT algorithm is used(i.e., SMFT or ESMFT), master process needs to add the failed process to $FailedProcsList$ while any process has any checkpoint data on the failed process's memory should perform a critical checkpoint to re-checked its tree to a the following available process (lines 17-21). After finishing the first iteration of FP-growth generation algorithm, failures should be recovered based on used $chk_schema$ (lines 26-30).



\begin{algorithm} [htp]
  \caption{\bf FT LFPTRee Generation}
\label{alg:generateLFPTree}
\begin{algorithmic}[1]
\State {\bf Input:} $L.Trans$, $G.Freq.List$, $\theta$, $chk\_schema$
\State initialization($chk\_schema$)
\State Let $L.Tree\leftarrow$ local FP-Tree (initially empty).
\For {each $T$ in $L.Trans$}
    \State $L.Tree$=merge($L.Tree$, $T$, $G.Freq.List$)

    \If{$Is\_Chk\_Iteration()$}
         \State performLFPChk($L.Tree$) //Normal Checkpoint
         \If{ $chk\_schema$==$SMFT$ OR $ESMFT$ }
            \State removeInvalidChks($MyChkslist$)
         \EndIf
    \EndIf

    \If{$Is\_TransChkPoint()$ AND $chk\_schema$==$ESMFT$}
        \State performTransChk($L.Trans$,$NoBackupProcs$)
    \EndIf
\If{A failure occurs in a process $P_f$}
        \State Master process adds $P_f.ID$ to $FailedProcsList$
        \If{$P_f\in MyChkslist$}
           \If{ $chk\_schema$==$SMFT$ OR $ESMFT$ }
                \State performLFPChk($L.Tree$) //Critical Checkpoint
                \State RemoveInvalidChks($MyChksList$)
           \EndIf
        \EndIf
    \EndIf
\EndFor
\State {\bf Recovery Block:}
\For{each $P_f$ in $FailedProcsList$}
  \State Master process broadcasts $P_f.ID$ to all other processes
  \State $L.Trans$=performRecovery($P_f$, $G.Freq.List$, $chk_schema$)
   \State generateLFPTree($L.Trans$, $G.Freq.List$, $\theta$, $chk\_schema$)
\EndFor
\end{algorithmic}
\end{algorithm}


==> text/design-knn.tex <==
\section{Proposed Fault Tolerant KNN Algorithm}
In this section, we present a parallel and fault-tolerant  KNN
algorithm.   The key feature of our approach is that one-sided
communication MPI-RMA  is used  to perform  periodic
checkpoints -- so that the cost of checkpointing is completely
overlapped with computation.

Recalling the baseline parallel KNN algorithm --  each sample from test
dataset has a corresponding list of nearest neighbors (in the form of a
priority queue $pq$) that needs to  be maintained throughout  the
execution.  The algorithm executes for $P$ iterations,  where $P$ is
also the number of  participating  processes. In  each iteration,
priority queues associated with each testing samples are updated, when a
``closer'' neighbor is found. Hence, priority queues are a critical data
structure, which is updated and must be saved for efficient recovery.

Using MPI-RMA technique, each node reserved a space that can handle a
checkpoint for a neighboring  node.  After processing local testing
samples, a complete checkpoint is performed by each process. Each
process uses  one-sided MPI communication to stores its local priority
queues on a neighboring node.

Algorithm~\ref{alg:KNN_alg} illustrates the checkpointing (and also the
recovery) procedure.  During the initialization procedure, each process
has its own $L.Trans.$ vector that contains local set of transactions
(line 1).  In line 2, each process $p_i$ defines a single vector, i.e.,
$metadata$  that represents a set of parameters to describe the status
of $L.Trans$ vector and checkpointed data stored on $p_i$ memory.  In
line 3, MPI-RMA is used to shared both vectors, i.e., $L.Trans.$ and
$meta-data$, to other processes.  Both $L. FPTree$ and remaining
transactions can be checkpointed using $performChk$ procedure.
Specific to this procedure, in  line 1, each process $P_i$ determines
its $TargetProcess$. For simplicity, we assume all processes
communicate in a ring fashion.  After this, process $p_i$ remotely
checks the available space on $p_{i+1}$ $L.Trans$ vector to decide
whether to only checkpoint its $L.FPTree$ or both $L.FPTree$ and
remaining $L.Trans$ or none of them (line 2-8).
\begin{algorithm} [htp]
\setstretch{1.0}
  \caption{\bf : FT K-Nearest Neighbor (KNN) Algorithm}
\label{alg:KNN_alg}
\begin{algorithmic}[1]
\Require {\bf Procedure: initialization}
\setcounter{ALG@line}{0}
\State $TargetProcess$ $\leftarrow$  $p_{i+1}$
\State Reserve memory space equals to $p_{i-1}$ current priority queues vector


\NoNumber\hrulefill
\NoNumber {\bf Procedure: performChk ($L.FPTree$, $L.Trans$)}
\setcounter{ALG@line}{0}
\For{$i$:1 to $P$}
\State send $L.S_{train}$ to process $p_{i+1}$
\State $L.S_{train}$ $\leftarrow$ receiveData($p_{i-1}$)
\For{each $m$ in $S_{test}$}
\For{each $n$ in $S_{train}$}
\State distance $\leftarrow$ calculateDistance($m$,$n$)
\State enqueue($pq_m$,$distance$)
\EndFor
\EndFor
\State {\bf Checkpoint $L.pq$ vector at $p_{i+1}$} //One-sided communication
\EndFor
\State



\NoNumber\hrulefill
\NoNumber {\bf Procedure: OPR-Recovery ($p_f$)}
\setcounter{ALG@line}{0}
\State $RecProcess$ $\leftarrow p_{f+1}$
\NoNumber {\bf Recovery process:}
\State  Merge ($p_f.pq$, $pq$)
\State  RecSamples $\leftarrow$ReadSamplesfromDisk($p_f$)



\NoNumber\hrulefill
\NoNumber {\bf Procedure: PPR-Recovery ($p_f$)}
\setcounter{ALG@line}{0}
\State $RecProcess$ $\leftarrow p_{f+1}$
\NoNumber {\bf Recovery process:}
\State  RecSamples $\leftarrow$ReadSamplesfromDisk($p_f$)
\State  Distribute($p_f.pq$)
\State  Distribute($RecSamples$)
\NoNumber {\bf All Processes:}
\State  Merge ($p_f.pq_i$, $L.pq$)
\State  Merge ($p_f.RecSamples_i$, $L.Samples$)
\end{algorithmic}
\end{algorithm}

For recovery, we  provide two different algorithms --  One Process
Recovery (OPR) and P-Processes Recovery (PPR).  As the name suggests,
in  OPR algorithm, only one process is used to recover and process  the
samples of the failed  process.  In comparison, the PPR algorithm uses
all of the remaining active processes to  process the workload of  the
failed process.

\noindent
{\bf OPR Recovery Algorithm:}
Assuming a failure occurs to a specific process $p_f$. The  master
process $p_m$ reads $p_f$ samples from the disk and send  it to the
recovery process $p_{f+1}$. Backup process $p_r$,  which already has the
priority queues of recovered samples,  assigns recovered priority queues
to the recovered samples. In the worst case, the recovery time
complexity is only associated  with retrieving the samples from the
disk, and is bounded by ($\frac{|T|}{|P|\cdot l}$).

\noindent
{\bf PPR Recovery Algorithm:}
In PPR recovery algorithm, all active nodes participate in the recovery
process. In the case of failure at process $p_f$,  the master process
$p_m$ re-reads the samples of $p_f$ from the disk and distribute them
among all available nodes  (with associated cost ($\frac{|T|}{|P|\cdot
b}$). The process $p_r$,  which has a back-up of priority queues
generated at the  process $p_f$, distributes the priority queues between
all available nodes. In this case, all active nodes have  the same
amount of samples to process.

The $performRecovery$ procedure from  Algorithm~\ref{alg:KNN_alg}  shows
the PPR recovery algorithm.   Assuming again ring communication between
the processes,  the recovery process will be the  process next to the
dead process $p_f$ in the ring (line 1). Overall, this process is used
to recover $p_f$ by merging latest checkpointed $p_f$ FP-Tree it has.
$p_f$ unprocessed transactions can  be recover from  {\em recovery
process} memory if it was checkpointed before failure or directly from
the disk  (line 3-7). Recovered transactions are re-distributed to
available processes to append them to their local transactions (line 8).

The time complexity of the recovery process in PPR algorithm is
$\frac{|T|}{|P|\cdot l}$ (time to reads samples from disk)+
$\frac{|T|}{|P|\cdot b}$ (time to re-distribute samples to available
nodes)+ $\frac{|T*K|}{|P|\cdot b}$ (time to distribute recovered
priority queues to available nodes).  Although the recovery time of PPR
algorithm is  higher  than the OPR algorithm, the total execution time
of KNN algorithm  supported  by PPR recovery algorithm is faster. This
is because PPR recovery algorithm ensures  load-balancing between
different  nodes even after recovery.







==> text/disclaimer.tex <==

\begin{disclaimer}

\end{disclaimer}


==> text/motivation.tex <==
\section{Motivation}
\label{sec:motivation}


==> text/spark-knn-eval.tex <==
\subsubsection{Comparison Against Spark}
Our FT-KNN system's efficiency   can also be shown by conducting a set of
experiments to compare it with KNN spark implementation.  In these set
of experiments, we use two real dataset (i.e., Ijcnn and Real-sim) for
comparison.

\begin{figure}[!htb]

 \subcaptionbox{Ijcnn Dataset
  \label{fig:a5}}
 {\includegraphics[width=1.6in,height=1.3in]{figs/spark-knn1.eps}}\hspace{0.7em}%
   \subcaptionbox{Real-sim Dataset
  \label{fig:a6}}
 {\includegraphics[width=1.6in,height=1.3in]{figs/spark-knn2.eps}}\hspace{0.7em}%

\caption{FT-based KNN Algorithm (Spark and MPI-based) with different support threshold $\theta$ and UCI Real Dataset}
 \label{fig:spark-knn}
\end{figure}

Figure~\ref{fig:spark-knn} illustrates the performance of both MPI-based
and Spark-based KNN implementations.  First, the execution time of
checkpointing algorithm in our MPI-based is much lower than  spark-based
implementation with a built-in checkpointing mechanism. Second, the
execution time difference between MPI-based and spark-based KNN
algorithm increases with larger number of cores. Finally, in the case of
failure, our PPR recovery algorithm's execution time  decreases with  increasing  number of
cores, whereas Spark-based KNN has less salability. 



